Using Semantic Information for Defining and Detecting OOD Inputs

As machine learning models continue to achieve impressive performance across different tasks, the importance of effective anomaly detection for such models has increased as well. It is common knowledge that even well-trained models lose their ability to function effectively on out-of-distribution inputs. Thus, out-of-distribution (OOD) detection has received some attention recently. In the vast majority of cases, it uses the distribution estimated by the training dataset for OOD detection. We demonstrate that the current detectors inherit the biases in the training dataset, unfortunately. This is a serious impediment, and can potentially restrict the utility of the trained model. This can render the current OOD detectors impermeable to inputs lying outside the training distribution but with the same semantic information (e.g. training class labels). To remedy this situation, we begin by defining what should ideally be treated as an OOD, by connecting inputs with their semantic information content. We perform OOD detection on semantic information extracted from the training data of MNIST and COCO datasets and show that it not only reduces false alarms but also significantly improves the detection of OOD inputs with spurious features from the training data.

==> algorithms.tex <==
\begin{minipage}[t]{0.48\textwidth}
\begin{algorithm}[H]
    \caption{ $\hat{\mathcal{D}}_I : $ \sout{OOD} Out-of-Intended Distribution Detection with Semantic Segmentation Network}
    \label{alg:sem_seg_ood_det}
    \begin{algorithmic}
        \STATE {\bfseries Input:} Test input $o \in \mathcal{X}$, 
        \STATE {\bfseries Parameters:} Semantic segmentation network $\mathcal{N}_s$ trained on $\mathcal{S}$, detection score $ds \in \{BS, OS\}$, detection threshold $\epsilon$
        \STATE {\bfseries Output:} ``$1$'' if $o$ is detected as OOD; ``$0$'' otherwise
        %\STATE $\hat{\mathcal{X}}_I = \{x^\prime\in\mathcal{X}:x^\prime=\mathcal{N}(x),x\in\mathcal{S}\}$
        \STATE $o'$ = $\mathcal{N}_s(o)$
        \STATE Create $z$ s.t, $z_{i,j}$ = $S(o'_{i,j})$, $ \forall i \in H, \forall j \in W$
        % \STATE $\hat{\mathcal{D}}_I$ = 
        % $\{\forall i \in h, \forall j \in w: S(x'[i][j])\}$ 
        % \STATE $v = \hat{\mathcal{D}}_I(\mathcal{N}(o))$ :\mathcal{X}\rightarrow\mathbb{R}^{h \times w \times 3}
        \STATE Return 1 if $ds(z) < \epsilon$, 0 otherwise 
    \end{algorithmic}
\end{algorithm}
\end{minipage} 
\hfill
\begin{minipage}[t]{0.48\textwidth}
\begin{algorithm}[H]
    \caption{ \sout{$\hat{\mathcal{D}}_I : $ OOD} Out-of-Intended Distribution Detection with \textcolor{blue}{Reference Set}}
    \label{alg:normal_ood_det}
    \begin{algorithmic}
        \STATE {\bfseries Input:} Test input $o \in \mathcal{X}$
        \STATE {\bfseries Parameters:} Segmentation algorithm $\mathcal{N}_r$, reference set $\mathcal{R}$, detection threshold $\epsilon$
        \STATE {\bfseries Output:} ``$1$'' if $o$ is detected as OOD; ``$0$'' otherwise
        \STATE $v = ComputeNearestSample(\mathcal{R}, \mathcal{N}_r(o))$
        {\color{red} MC: unclear here; perhaps you meant $v_i=ComputeNearestSample(r_i,\mathcal{N}_r(o))$, $r_i\in\mathcal{R}$}
        \STATE Return 1 if $\max(v) < \epsilon$, 0 otherwise 
        {\color{red} MC: continuing from above, perhaps here you meant ``Return 1 if $\max_i(v_i) < \epsilon$, 0 otherwise''}
    \end{algorithmic}
\end{algorithm}
\end{minipage}
